Neural architecture impact on identifying temporally extended Reinforcement Learning tasks

Inspired by recent developments in attention models for image classification and natural language processing, we present various Attention based architectures in reinforcement learning (RL) domain, capable of performing well on OpenAI Gym Atari-2600 game suite. In spite of the recent success of Deep Reinforcement learning techniques in various fields like robotics, gaming and healthcare, they suffer from a major drawback that neural networks are difficult to interpret. We try to get around this problem with the help of Attention based models. In Attention based models, extracting and overlaying of attention map onto images allows for direct observation of information used by agent to select actions and easier interpretation of logic behind the chosen actions. Our models in addition to playing well on gym-Atari environments, also provide insights on how agent perceives its environment. In addition, motivated by recent developments in attention based video-classification models using Vision Transformer, we come up with an architecture based on Vision Transformer, for image-based RL domain too. Compared to previous works in Vision Transformer, our model is faster to train and requires fewer computational resources. 3

==> chapters/analysis.tex <==
We performed various analysis on our architectures to come up with the optimum network design and hyper parameters. In the following sections, we present some of the analysis and impact of network design decisions. \\[0.1in]
Training steps per second (SPS), approximately calculated as $\texttt{SPS} = \texttt{total\textunderscore{steps}}/\texttt{training\textunderscore{time}}$ is considered a measure of training speed. We performed most of our analysis on OpenAI Gym \cite{brockman2016openai} Atari-2600 Pong, and Enduro environments. Besides average episode returns and episode lengths, other metrics considered are: training speed (SPS), total training duration, total network-parameter size and inference time. Inference time is defined as the time lapsed between two consecutive agent steps. Episode return and length are computed as moving average over last 100 episodes. Inference time is observed and averaged over an episode.

\section{Impact of using ResNet in Vision Core}
We experimented with both a smaller convolutional network (ConvNet) as well the larger ResNet (Figure \ref{fig:resnet_architecture}) in vision core for Mott architecture (Section \ref{sec:motts_architecture_section}). The model with ResNet was bigger in terms of parameter volume and learned faster in terms of training steps, compared to ConvNet(Figure \ref{fig:motts_resnet_frame_stacking_impact} Left). Since there is significant improvement in learning speed with ResNet, for all future architectures, we decided to go ahead with ResNet(Figure \ref{fig:resnet_architecture}). Both networks were trained for 40M steps with similar hyper parameters. Findings are summarized in the table [\ref{tab:resnet_vs_convnet}].

\begin{table}[hbt!]
    \caption{Comparison of performance metrics between ResNet and Convnet models trained on Atari-Enduro environment for 40M steps.}
    \centering
        \begin{tabular}{p{4cm}|p{1.5cm}|p{1.5cm}}
         Metric & ResNet & ConvNet\\
         \hline \hline
         total parameter size   & 2.18M    & 2.01M\\
         total training time &   11.70h  & 6.20h\\
         training speed (SPS) &   949.27  & 1791.16\\
         inference time per cycle & 40.4ms & 18.84ms\\
        \end{tabular}
    \label{tab:resnet_vs_convnet}
\end{table}

\section{Impact of pre-processing technique: frame stacking}
A common pre-processing technique proposed in Mnih et al.\cite{Mnih2015}, involves downsizing images, converting them to grey scale and stacking last $m$ frames along channel dimension such that observation space \textbf{X} \in $ \mathbf{R}^{H \times W \times m}$ with $m = 4$. To analyse impact of frame stacking, two experiments: one with frame stacking with $m=4$ and other without frame stacking such that $m=1$, was run on Mott architecture (Section \ref{sec:motts_architecture_section}). Both model were trained for 40M steps on Atari-Enduro environment. Frame stacking clearly speeds up learning as seen from the performance curves (Figure \ref{fig:motts_resnet_frame_stacking_impact} Right). 

\begin{figure}[hbt!]
\centering
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/non_vit_results/resnet_convnet_epi_returns.png}
    \label{fig:mean_returns_resnet_vs_convnet}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/non_vit_results/frame_stacking_episode_returns.png}
    \label{fig:mean_returns_frame_stacking}
\end{subfigure}%

\caption{Left: Impact of using ResNet in Vision core. Right: Impact of frame stacking pre-processing technique.}
\label{fig:motts_resnet_frame_stacking_impact}
\end{figure}

\section{Effect of varying number of decoder layers in Adaptive architecture}
\label{sec:effect_num_layers_transformer}
We varied the number of decoder layers from 1 to 3 for Adaptive architecture(Section \ref{sec: adaptive_transformer_xl}) on Pong environment trained for 10M steps. Contrary to expectation, increasing the number of layers did not significantly improve the convergence speed, in spite of increasing network capacity. In fact, we noticed that architecture with one and two layers converged faster than the three layers variant(Figure \ref{fig:effect_num_layers_transformer}). We believe that the reason is reactive environments like Pong where time dependencies do not exceed more than 100 time-steps, are not sufficiently memory intensive to fully utilize the Transformer's memory capabilities. As the number of layers increase, total model parameters increases and result in both slower training and inference times(Table \ref{tab:variation_layers_transformer}). Peak in episode-length curve(Figure \ref{fig:effect_num_layers_transformer} Right) represents the training instant where the opponent cpu-agent is able to prolong the game duration by scoring points against the model agent, thereby extending the episode duration. Once the model figures out the optimum move, episode steps are brought down with cpu-agent loosing 0-21 every time thereafter.

\begin{table}[hbt!]
    \centering
    \caption{Effect of variation of number of decoder-layers in Adaptive architecture(Section \ref{sec: adaptive_transformer_xl}) trained for 10M steps.}
        \begin{tabular}{p{4cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
         Metric & Layers 1 & Layers 2 & Layers 3\\
         \hline \hline
         total parameter size   & 1.92M  & 2.77M  & 3.63M\\
         total training time &   2.57h  & 3.32h  & 4.02h\\
         training speed (SPS) &   1080.26  & 834.65  & 691.12\\
         inference time per cycle & 14.84ms & 17.46ms & 19.87ms\\
        \end{tabular}
    \label{tab:variation_layers_transformer}
\end{table}

\begin{figure}[hbt!]
\centering
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/non_vit_results/num_layers_episode_returns.png}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/non_vit_results/num_layers_episode_lens.png}
\end{subfigure}%

\caption{The models \texttt{layer-1}, \texttt{layers-2} and \texttt{layers-3} converge with decreasing speeds with \texttt{layers-3} being the slowest.}
\label{fig:effect_num_layers_transformer}
\end{figure}

\section{Effect of scaling images to [0, 1]} 
In this section, we analyze the impact of value normalization technique in which images are scaled from $(0,255)$ to $(0,1)$. To observe the effect of scaling, two Adaptive architecture models: one with and other without rescaling were tested. Surprisingly, a slight drop in performance is observed in the rescaled case compared to nonscaled ones (Figure \ref{fig:effect_scaling_by_255}). Hence, for all future experiments we decided not to use rescaling. \\[0.1in]

\begin{figure}[hbt!]
\centering
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/non_vit_results/effect_scaling_ret.png}
    \label{fig:effect_scaling_returns}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/non_vit_results/effect_scaling_loss.png}
    \label{fig:effect_scaling_loss}
\end{subfigure}%

\caption{Impact of scaling images to $(0,1)$ on models trained for 10M steps with Adaptive architecture (Section \ref{sec: adaptive_transformer_xl}).}
\label{fig:effect_scaling_by_255}
\end{figure}

\section{TimeSformer architecture: Effect of patch size variation}
In TimeSformer variant(Section \ref{sec:timesformer_method}), each frame is decomposed into \textbf{N} non-overlapping patches of size $P \times P$. Total number of patches per frame is given by $N = HW / P^2$. We experimented with three different patch values: 7, 14 and 28 on Pong environment for 60M steps on Divided Space-Time architecture (Figure \ref{fig:vit_attention_scheme} Right). Decreasing patch size would result in more spatial granularity but increases effective sequence length, leading to an increase in training time(Table \ref{tab:vit_patch_size_variation}). In terms of number of training steps, learning speed decreases with an increase in patch size. For instance, patch-size: 7 model learns the fastest, followed by 14, and 28 being the slowest (Figure \ref{fig:patch_frame_size_impact} Left). With patch-size 28, image is split into just 9 patches and the agent might be loosing valuable pixel information in coarse patch embedding operation. We have chosen patch size 7 for further experiments for better attention-visualisation and spatial resolution. \\[0.1in]

\begin{table}[hbt!]
    \caption{Impact of patch size variation in ViT Divided Space-Time model for Pong environment.}
    \centering
        \begin{tabular}{p{4cm}|p{2cm}|p{2cm}|p{2cm}}
         Metric & patch-size 7 & patch-size 14 & patch-size 28\\
         \hline \hline
         total parameter size & 0.589M    & 0.166M    & 0.095M\\
         total training time &  7.24h    & 3.60h    & 2.60h\\
         training speed (SPS) & 2301.22  & 4627.01  & 6432.63\\
         inference time per cycle & 6.8ms & 3.3ms & 2.64ms\\
        \end{tabular}
    \label{tab:vit_patch_size_variation}
\end{table}


\begin{figure}[hbt!]
\centering
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/vit_results/patch_size_effect.png}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/vit_results/frame_shape_effect.png}
\end{subfigure}%
\caption{Impact of patch size(Left) and frame size variation(Right) for TimeSformer Divided Space-Time model(Section \ref{sec:timesformer_method}) in Pong environment.}
\label{fig:patch_frame_size_impact}
\end{figure}

\section{TimeSformer architecture: Effect of environment size variation}
\label{sec:vit_env_size_impact}
Following the preprocessing techniques used in Mnih et al. \cite{Mnih2015}, we downsize, convert to gray scale and frame-stack the last 4 RGB Atari frames from $(210 \times 160 \times 3)$ to $(84 \times 84 \times 4)$. Higher image resolution results in more number of patches and thus longer sequence length(N) per frame. We additionally experimented with frame sizes 42 and 21 using Divided Space-Time model(Figure \ref{fig:vit_attention_scheme} Right). Training time increases with environment size since time complexity for Divided Space-Time model scales with $(N + F)$ (Table \ref{tab:vit_env_size_impact}). The impact is more profound for Joint Space-Time attention model (Figure \ref{fig:vit_attention_scheme} Left) where the run time directly scales with $(N \times F)$. Hence down-scaling from $(84 \times 84)$ to $(42 \times 42)$ sped up training tremendously for Joint Space-Time attention model (Figure \ref{fig:vit_attention_scheme} Left). The increase in total parameter size with environment size is due to the growth of parameter volume of Linear layer following Policy-core (Section \ref{sec:timesformer_method}). The Linear layer is responsible for flattening and shrinking Policy core output to a lower-dimensional space. Hence, the total parameter size of Linear layer scales quadratically with the environment size. Also, the training performance deteriorated on reducing the environment shape to $(21 \times 21)$ (Figure \ref{fig:patch_frame_size_impact} Right).

\begin{table}[hbt!]
    \caption{Impact of variation in environment frame shape for Divided Space-Time architecture (Figure \ref{fig:vit_attention_scheme} Right)}
    \centering
        \begin{tabular}{p{4cm}|p{2cm}|p{2cm}|p{2cm}}
         Metric & env-size 21 & env-size 42 & env-size 84\\
         \hline \hline
         total parameter size   & 0.11M    & 0.22M & 0.56M\\
         total training time &   2.36h  & 3.68h  & 7.61h\\
         training speed (SPS) &   4696.37  & 3018.12  & 1459.69\\
         inference time per cycle & 4.5ms & 6.5ms & 17ms\\
        \end{tabular}
    \label{tab:vit_env_size_impact}
\end{table}

\section{TimeSformer architecture: Effect of Hybrid architecture}
Similar to Hydrid architecture used in ViT (Section \ref{sec:vision_transformer_background}), we compare the effect of using ResNet \cite{DBLP:journals/corr/HeZRS15} and a single-layer 2D-convolutional(ConvNet) network similar to TimeSformer model \cite{DBLP:journals/corr/abs-2102-05095} to generate image-patches sequences. Similar to the trends observed in Mott (Figure \ref{fig:motts_resnet_frame_stacking_impact} Left), significant improvement in training performance has been observed with ResNet \cite{DBLP:journals/corr/HeZRS15} configuration (Figure \ref{fig:vit_resnet_convnet_embsize_impact} Left). Hence for all subsequent experiments, we used ResNet as the patch-embedding network. However, the improvement in training performance comes with a price of increase in total training time and slower inference (Table \ref{tab:vit_effect_resnet}). Another interesting observation here is that the total parameter size is more for ConvNet based model compared to ResNet based model, even though ResNet (\ref{fig:resnet_architecture}) is more parameter intensive that the single layer CNN. Similar to observation in Section \ref{sec:vit_env_size_impact}, this is again attributed to substantial increase in the parameter size of the Linear layer responsible for shrinking Policy core's output. Output frame size of ConvNet layer is $(12 \times 12)$ whereas it is $(11 \times 11)$ for ResNet. Since size of the mapping Linear layer scales quadratically with the output frame size, this leads to Hybrid architecture using ResNet having fewer parameters than the normal architecture using ConvNet.

\begin{table}[hbt!]
    \caption{Impact of Hydrid architecture with ResNet compared to normal convolutional network for Divided Space-Time model.}
    \centering
        \begin{tabular}{p{4cm}|p{2cm}|p{2cm}}
         Metric & ConvNet & ResNet\\
         \hline \hline
         total parameter size   & 0.59M    & 0.56M\\
         total training time &   4.84h  & 7.61h\\
         training speed (SPS) &   2294.42  & 1459.7\\
         inference time per cycle & 6.5ms & 17ms\\
        \end{tabular}
    \label{tab:vit_effect_resnet}
\end{table}

\begin{figure}[hbt!]
\centering
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/vit_results/effect_resnet.png}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/vit_results/effect_emb_size.png}
\end{subfigure}%
\caption{Impact of using ResNet as patch embedding network(Left) and variation of \texttt{emb\textunderscore{size}}(Right) for TimeSformer Divided Space-Time model(Section \ref{sec:timesformer_method}) with Pong environment.}
\label{fig:vit_resnet_convnet_embsize_impact}
\end{figure}


\section{TimeSformer architecture: Effect of embedded dimension for Patch embedding network}
Patch Embedding network encodes input frame $X$ \in $ \mathbf{R}^{H \times W \times C}$ to $X'$ \in $ \mathbf{R}^{h \times w \times emb\textunderscore{size}}$ which are in turn flattened to $X''$ \in $ \mathbf{R}^{N \times P^2 \times emb\textunderscore{size}}$. Hyper parameters \texttt{emb\textunderscore{size}} determines latent space size of encoded input frame. Increasing \texttt{emb\textunderscore{size}} increases network capacity at the expense of training time. We experimented with values: $[8, 16, 32, 64]$ for \texttt{emb\textunderscore{size}} on Pong environment for 40M training steps. Training time increases significantly with higher values of \texttt{emb\textunderscore{size}} with no proportionate improvement in returns or learning speed (Table \ref{tab:vit_emb_dim_variation} and Figure \ref{fig:vit_resnet_convnet_embsize_impact} Right). We have tuned \texttt{emb\textunderscore{size}} to 16 to trade-off training speed and model capacity for our subsequent experiments. \\[0.1in]

\begin{table}[hbt!]
    \caption{Impact of variation in \texttt{emb\textunderscore{size}} for Divided Space-Time model with Pong environment.}
    \centering
        \begin{tabular}{p{4cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
         Metric & emb-8 & emb-16 & emb-32 & emb-64\\
         \hline \hline
         total parameter size & 0.30M  & 0.56M & 1.09M & 2.24M\\
         total training time & 6.33h  & 7.64h  & 11.36h & 17.89h\\
         training speed (SPS) &  1754.24 & 1459.69 & 977.55 & 620.86\\
         inference time per cycle & 13.5ms & 16ms & 21.5ms & 33.5ms\\
        \end{tabular}
    \label{tab:vit_emb_dim_variation}
\end{table}


\section{TimeSformer architecture: Effect of varying number of attention layers}
Similar to Adaptive architecture experiment (Section \ref{sec:effect_num_layers_transformer}), we varied \texttt{num\textunderscore {layers}} in $[1, 2, 3, 4]$. Increasing the number of layers slightly increased the total parameter size with minor improvement in agent performance (Table \ref{tab:vit_effect_num_layers_observations} and Figure \ref{fig:num_layers_div_join_comparison} Left). This trend is similar to that observed with the Adaptive architecture (Figure \ref{fig:effect_num_layers_transformer}) and could be again attributed to less memory-intensive nature of Atari-Pong environment. Also, adding layers significantly slowed down both training and inference. For all later experiments, we used a single-layer configuration. \\[0.1in]


\begin{table}[hbt!]
    \caption{Impact of variation in number of attention layers in TimeSformer model (Section \ref{sec:timesformer_method}) for Pong environment.}
    \centering
        \begin{tabular}{p{4cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
         Metric & layers:1 & layers:2 & layers:3 & layers:4\\
         \hline \hline
         total parameter size & 0.5589M  & 0.5635M & 0.5681M & 0.5727M\\
         total training time & 7.64h  & 10.23h  & 12.63h & 16.15h\\
         training speed (SPS) &  1459.69 & 1086.69 & 879.5 & 688.0\\
         inference time per cycle & 16ms & 22.5ms & 29ms & 35ms\\
        \end{tabular}
    \label{tab:vit_effect_num_layers_observations}
\end{table}


\begin{figure}[hbt!]
\centering
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/vit_results/effect_num_layers.png}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{images/analysis_ground/vit_results/div_joint_sp_time.png}
\end{subfigure}%
\caption{Effect of varying number of attention layers(Left) and performance comparison between Divided Space-Time and Joint Space-Time TimeSformer(Section \ref{sec:timesformer_method}) agents trained on Pong environment.}
\label{fig:num_layers_div_join_comparison}
\end{figure}

\section{TimeSformer architecture: Comparison between Divided and Joint Space-Time models}
\label{sec:divided_vs_joint_space_time}
We compare training time and performance characteristics for Divided Space-Time and Joint Space-Time architectures. As mentioned in previous Section \ref{sec:timesformer_theory}, training time of Joint Space-Time agents is of order $\mathcal{O}(N \times F)$, whereas for Divided Space-Time agents, it reduces to $\mathcal{O}(N + F)$, where $N$ represents number of patches per image and $F$ number of frames considered. For both attention schemes, we are considering two models: first one with environment shape $(84 \times 84)$ and second with reduced shape $(42 \times 42)$. Faster training was observed with reduced environment shapes for both Divided and Joint Space-Time models (Table \ref{tab:vit_div_joint_space_time_observations}). Learning performance wise (Figure \ref{fig:num_layers_div_join_comparison} Right), there was no significant difference between the models. All models were trained on Pong environment for 20M steps. Computation wise, it is expensive to run the Joint Space-Time models without environment resizing. \\[0.1in]

\begin{table}[hbt!]
    \caption{Performance comparison of Divided Space-Time and Joint Space-Time agents.}
    \centering
        \begin{tabular}{p{2.5cm}|p{2.0cm}|p{2.0cm}|p{2.0cm}|p{2.0cm}}
         Metric & divided-42 & divided-84 & joint-42 & joint-84\\
         \hline \hline
         total params & 0.221M & 0.5589M  & 0.2165M & 0.5565M\\
         training time & 1.87h & 3.81h  & 3.17h  & 21.12h\\
         SPS & 3018.12 & 1460.06 & 1750.70 & 263.1\\
         inference time & 4.5ms & 16ms & 9.5ms & 81.5ms\\
        \end{tabular}
    \label{tab:vit_div_joint_space_time_observations}
\end{table}

%%%%%%%%%%%%%%%% end of Analysis section %%%%%%%%%%%%%%%%
%% current status:
%% writing done: .
%% proof reading done: 22-Aug-21
%% Review by RR done: 
%% total number of pages: 10 (27-34)
%% RR review points addressed: 4-Sept-21
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
